GPT-4 as an Agronomist Assistant? Answering Agriculture Exams Using Large Language Models

Large language models (LLMs) have demonstrated remarkable capabilities in natural language understanding across various domains, including healthcare and finance. For some tasks, LLMs achieve similar or better performance than trained human beings, therefore it is reasonable to employ human exams (e.g., certification tests) to assess the performance of LLMs. We present a comprehensive evaluation of popular LLMs, such as Llama 2 and GPT, on their ability to answer agriculture-related questions. In our evaluation, we also employ RAG (Retrieval-Augmented Generation) and ER (Ensemble Refinement) techniques, which combine information retrieval, generation capabilities, and prompting strategies to improve the LLMs' performance. To demonstrate the capabilities of LLMs, we selected agriculture exams and benchmark datasets from three of the largest agriculture producer countries: Brazil, India, and the USA. Our analysis highlights GPT-4's ability to achieve a passing score on exams to earn credits for renewing agronomist certifications, answering 93% of the questions correctly and outperforming earlier general-purpose models, which achieved 88% accuracy. On one of our experiments, GPT-4 obtained the highest performance when compared to human subjects. This performance suggests that GPT-4 could potentially pass on major graduate education admission tests or even earn credits for renewing agronomy certificates. We also explore the models' capacity to address general agriculture-related questions and generate crop management guidelines for Brazilian and Indian farmers, utilizing robust datasets from the Brazilian Agency of Agriculture (Embrapa) and graduate program exams from India. The results suggest that GPT-4, ER, and RAG can contribute meaningfully to agricultural education, assessment, and crop management practice, offering valuable insights to farmers and agricultural professionals.

==> Makefile <==
PWD = $(shell pwd)

TEXINPUTS = ${PWD}:
BSTINPUTS = ${PWD}:

SETENVVAR = \
			BSTINPUTS="${BSTINPUTS}" \
			TEXINPUTS="${TEXINPUTS}"

SOURCE_FILES = $(wildcard *.tex *.bib)

BIBTEX = ${SETENVVAR} bibtex
LATEXMK = ${SETENVVAR} latexmk
PDFLATEX = ${SETENVVAR} pdflatex -shell-escape --synctex=1

.PHONY: clean

all: paper.pdf

paper.pdf: ${SOURCE_FILES}
	${PDFLATEX} paper.tex
	${BIBTEX} paper
	latex_count=6 ; \
	while egrep -s 'Rerun (LaTeX|to get cross-references right)' paper.log && [ $$latex_count -gt 0 ] ;\
		do \
			echo "Rerunning latex..." ;\
			${PDFLATEX} paper.tex ;\
			latex_count=`expr $$latex_count - 1` ;\
		done
	${BIBTEX} paper
	${PDFLATEX} paper.tex


clean:
	rm -f *.aux *.auxlock *.dvi *.lof *.lot *.lox *.toc *.bbl *.blg *.blf *.pyc *.bak *.log *.out *.fls *.fdb_latexmk *_latexmk *.synctex.gz paper.pdf

